Word Sense Induction with Knowledge Distillation from BERT

Pre-trained contextual language models are ubiquitously employed for language understanding tasks, but are unsuitable for resource-constrained systems. Noncontextual word embeddings are an efficient alternative in these settings. Such methods typically use one vector to encode multiple different meanings of a word, and incur errors due to polysemy. This paper proposes a two-stage method to distill multiple word senses from a pre-trained language model (BERT) by using attention over the senses of a word in a context and transferring this sense information to fit multi-sense embeddings in a skip-gram-like framework. We demonstrate an effective approach to training the sense disambiguation mechanism in our model with a distribution over word senses extracted from the output layer embeddings of BERT. Experiments on the contextual word similarity and sense induction tasks show that this method is superior to or competitive with state-of-the-art multi-sense embeddings on multiple benchmark data sets, and experiments with an embedding-based topic model (ETM) demonstrates the benefits of using this multi-sense embedding in a downstream application.

==> exps_bak.tex <==
\section{Experiments}
We conduct both qualitative and quantitative experiments on our trained sense embedding model.
In this section, the dataset and training procedure is discussed first.
Then, we look at the nearest neighbours of words in context and the performance of our sense embeddings models on 2 tasks.
We also look at the quality of our two-stage knowledge distillation method.

\subsection{Dataset and Traning}
We trained our models on the April 2010 snapshot of Wikipedia \cite{shaoul2010wiki} for fair comparison with the previous multi-sense embedding models. 
This corpus has over 2 million documents and about 990 million words.
We also used the same vocabulary set as \citet{neelakantan2014efficient} containing  99,081 words.
During preprocessing, we use the python library \textit{nltk}'s word tokenizer and filter out tokens that do not contain any alpha-numeric characters.

We selected the hyperparameters of our models by training them on a small part of the corpus based on the loss value on a validation set.
For training, we set the context window size to $\Delta = 5$ and slide this window over each paragraph in the document.
So the context window does not overlap between paragraphs but can go over sentence boundaries in a paragraph. 
We use 10 negative samples for each positive (word, context) pair.
We do not apply subsampling like \texttt{word2vec} since the BERT model was pre-trained on sentences without subsampling.
We train 3 sense embeddings for each word following prior work \cite{neelakantan2014efficient}.
The embedding dimension is set to 300 for comparison with prior work.
The embeddings $\mathbf{v}$, $\mathbf{d}$, $\mathbf{g}$ and $\mathbf{u}$ are initialized with uniform distribution between $[-1/D, 1/D]$ where $D$ is the embedding dimension.
We use the Adam \cite{kingma2014adam} optimizer with a learning rate of $0.001$.

The base model of BERT is used as the pre-trained language model which is a transformer with 12 layers and 768 dimensional embeddings in each layer. 
The PyTorch \textit{transformers} \cite{wolf2019huggingface} library is used for inference through the BERT-base model.
So, the intermediate sense embeddings in the BERT sense model have dimension of 768.
There are a total of about $720M$ context windows in full wikipedia corpus. 
With a batch size of 2048, it takes about 10 hours to train the sense embedding model on the wikipedia corpus for one epoch in a Tesla V100 gpu.
Training the sense embedding model with knowledge distillation requires inference through the pre-trained BERT model. 
With 16 Tesla V100 gpus, it takes about 20 hours for one epoch of knowledge distillation with a total batch size of 8192.
As it is expensive to run inference through the pre-trained BERT model, we train the Bert sense model over $180M$ context windows for 5 epochs.
The sense embedding models with and without knowledge distillation are trained for 2 epochs over the full Wikipedia dataset.
The weight for the knowledge distillation loss (Eq. \ref{eq:transfer_loss}) $\alpha=1$ is selected from \{0.1, 0.5, 1.0\}.
Temperature parameter $T$ is set to 4 by tuning over the range [2,6].


\subsection{Nearest Neighbours}
The nearest neighbours of words in context are shown in Table \ref{tab:nn}.
Given the context words, the context embedding is computed using Eq. \ref{eq:c-iter} and sense probability distribution is computed with Eq. \ref{eq:sensealpha}.
The most probable sense is selected and then the cosine distance is computed with the global embeddings of all words in the vocabulary.
Table \ref{tab:nn} also shows the values of the sense probability for the word in context.
The sense probabilities are close to 1 in most of the cases.
This indicates that the model learned a narrow distribution over the senses and it selects a single sense most of the time even though there was no penalty against a flat distribution in the loss function.

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{c|c|c} \hline
         Context & Sense: Prob. & Nearest Neighbours \\ \hline \hline
         macintosh is a family of computers from \textit{apple} & $1: 0.99$ & apple, amstrad, macintosh, commodore, dos \\ \hline
         \textit{apple} software includes mac os x & $2 : 0.963$ & microsoft, ipod, announced, software, mac \\ \hline
         \textit{apple} is good for health & $3: 0.999$ & apple, candy, strawberry, cherry, blueberry \\ \hline \hline
         the power \textit{plant} is closing & $3: 1.0$ & mill, plant, cogeneration, factory, mw \\ \hline
         the science of \textit{plant} life & $2:  1.0$ & species, plant, plants, lichens, insects \\ \hline
         the seed of a \textit{plant} & $1 : 0.99$ & thistle, plant, gorse, salvia, leaves \\ \hline \hline
         the \textit{cell} membranes of an organism & $3 : 1.0$ & depolarization, contractile, hematopoietic, follicular, apoptosis \\ \hline
         almost everyone has a \textit{cell} phone now & $2 : 0.99$ & phone, cell, phones, mobile, each \\ \hline
         prison \textit{cell} is not a pleasant place & $1 : 0.99$ & prison, room, bomb, arrives, jail \\ \hline \hline
         the creek flowed over solid \textit{rock} & $1: 0.54$ & station, pinned, creek, park, mika \\ \hline
         they collected \textit{rock} samples from the site & $2 : 0.99$ & rocks, sandstone, volcanic, granite, outcrops \\ \hline
         many bands are playing in this \textit{rock} concert & $3 : 0.99$ & band, rock,  lo-fi, punk, pop \\ \hline
    \end{tabular}
    \caption{Top 5 nearest neighbours of words in context based on cosine similarity. We also report the index of the selected sense and its probability in that context.}
    \label{tab:nn}
\end{table*}

\subsection{Word Sense Induction}
Word sense embedding models learn to assign the correct meaning to a word in context. 
This is directly related to the Word Sense Induction (WSI) task where the goal is to identify different meanings of a word in different contexts.
This task evaluates the model's ability to select the appropriate sense given a context.
For assigning a sense to a word in context, we take the words in its context window (size 5) and compute the context embedding using Eq. \ref{eq:c-iter}.
Then the sense probability from Eq. \ref{eq:sensealpha} gives the most probable sense for that context.

We follow \citet{bartunov2016breaking} for the evaluation dataset and clustering measures.
Three WSI datasets are used in our experiments.
Each dataset consists of a collection of words with different contexts for each word.
The task is to assign a meaning to each context of a word.
The SemEval-2007 dataset is from SemEval-2007 Task 2 competition \cite{agirre-soroa-2007-semeval}.
It contains 27232 contexts for 100 words collected from Wall Street Journal (WSJ) corpus.
The SemEval-2010 dataset is from the SemEval-2010 Task 14 competition \cite{manandhar-klapaftis-2009-semeval} which contains 8915 contexts for 100 words. 
Finally, the SemEval-2013 dataset comes from the SemEval-2013 Task 13 \cite{jurgens-klapaftis-2013-semeval} with 4664 contexts for 50 words.

The human annotations in these datasets may contain more or less meanings than the fixed number of senses in the model.
For evaluation, we cluster the different contexts of a word according to the model's predicted sense and the human annotated sense.
So the scoring measure is essentially a clustering evaluation method.
To evaluate the clustering of of a set of points, we take pairs of points in the dataset and check if they are in the same cluster according to the ground truth.
For the SemEval competitions, two traditional metrics were used: F-score and V-measure.
But there are intrinsic biases in these methods. 
F-score will be higher for a cluster with fewer centers while V-measure will be higher for clusters with a large number of centers.
So \citet{bartunov2016breaking} used the ARI (Adjusted Rand Index) as the clustering evaluation method since it does not suffer from these problems.

In Table \ref{tab:wsi}, multi-sense models used for comparison are: Multi-Sense Skip-gram model (MSSG) \cite{neelakantan2014efficient} which uses a clustering mechanism for different senses,   Multi-prototype Skip-gram model (MPSG) \cite{tian2014probabilistic} that uses an EM algorithm to learn the clusters, AdaGram \cite{bartunov2016breaking}, a Bayesian model trained with stochastic variational inference, MUSE \cite{lee2017muse}, a sense embedding model learned in a reinforcement learning framework  and Disambiguated skip-gram \cite{grzegorczyk-kurdziel-2018-disambiguated} which uses Gumbel-softmax and entropy loss. 
Single-sense models like skip-gram cannot be used in this task since the task is to assign different senses to different contexts of a word.
We report the ARI scores for MSSG, MPSG and AdaGram from \citet{bartunov2016breaking}.
Disambiguated skip-gram results are collected from \citet{grzegorczyk-kurdziel-2018-disambiguated}.
We used the trained weights from MUSE with Boltzmann method \cite{lee2017muse} for this task.

The MUSE model modularizes the sense selection and sense representation tasks.
This shows strong performance in word similarity tasks (section \ref{sec:scws}) but fails to induce meaningful senses given a context.
The Disambiguated Skip-gram model was the best model on SemEval-2007 and SemEval-2010 datasets.
This model uses Gumbel-softmax to improve the gradient propagation through the distribution over the senses of a word in context.
Our sense embedding model performs better than MSSG and MPSG models but there is a large gap with the state-of-the-art.
We can see a significant improvement in ARI score ($2-3x$) on the 3 datasets with knowledge distillation from BERT.
This shows the effectiveness of extracting the knowledge in the contextual embeddings from pre-trained language models like BERT.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c} \hline
    Model & SE-2007 & SE-2010 & SE-2013 \\ \hline
    MSSG & $0.048$ & $0.085$ & $0.033$ \\
    MPSG & $0.044$ & $0.077$ & $0.033$ \\
    AdaGram & $0.069$ & $0.097$ & $0.061$ \\
    MUSE & $0.0009$ & $0.01$ & $0.006$ \\ 
    Disamb. SG & $0.077$ & $0.117$ & $0.045$ \\ \hline \hline
    SenseEmbed & $0.053$ & $0.076$ & $0.054$ \\
    BertSense & $0.179$ & $0.179$ & $0.155$ \\
    BertKDEmbed & $\mathbf{0.145}$ & $\mathbf{0.144}$ & $\mathbf{0.133}$ \\ \hline
    \end{tabular}
    \caption{ARI (Adjusted Rand Index) scores for word sense induction tasks. This is the average score over all words in the test set. All models in this table have multiple embeddings per word with dimension of 300. The Adagram and Disambiguated skip-gram learn variable number of sense while all other models learn fixed number of senses per word. All baseline results except MUSE were collected from \cite{grzegorczyk-kurdziel-2018-disambiguated}. Our embedding model with knowledge distillation scores much higher than the previous best.}
    \label{tab:wsi}
\end{table}

\subsection{Contextual Word Similarity}
\label{sec:scws}
To evaluate the representation of word senses learned by our model, we use the contextual word similarity task where a pair words in two paragraphs are given. 
The task is to predict the similarity of the meaning of these 2 words given the context they were used.
We use the Stanford Contextual Word Similarity (SCWS) dataset \cite{huang2012improving} for this purpose.
This dataset contains 2003 word pairs with their contexts, selected from Wikipedia.
Each word pair has 10 human annotation scores between 1 to 10. 
The average of these scores are used as the similarity score for a word pair.
Spearman's rank correlation $\rho$ is used to measure the degree of agreement between the human similarity score and the model's similarity score.

We use the following methods for predicting similarity of two words in context based on the sense embedding model \cite{reisinger2010multi}: AvgSimC and MaxSimC.
The AvgSimC measure weighs the cosine similarity of all combinations of sense embeddings of 2 words with the probability of those 2 senses given their respective contexts.
\begin{align}
\begin{split}
    AvgSimC & (w_1,w_2) = \\ &\frac{1}{K^2} \sum_{i=1}^K \sum_{j=1}^K p(w_1=w_1^i|w_1,C) \\ &p(w_2=w_2^j|w_2,C) cos(v_{1}^i, v_{2}^j)
\end{split}
\end{align}
Here, the cosine similarity between sense $i$ word 1 and sense $j$ of word 2 is multiplied by the probability these 2 senses given their contexts. 
Finally, the average over all combinations of senses are taken.

The MaxSimC method selects the best sense for each context based on their probabilities and calculates their cosine similarity.
\begin{equation}
    MaxSimC(w_1,w_2) = cos(v_{1}^i, v_{2}^j)
\end{equation}
where 
\begin{align}
\begin{split}
i = \arg\max_{k=1}^K p(w_1=w_1^k|w_1,C) \\
j = \arg\max_{k=1}^K p(w_2=w_2^k|w_2,C)
\end{split}
\end{align}

For comparison with baselines on this task, we use the single-sense skip-gram model \cite{mikolov2013distributed} with 300 and 900 dimensions since our word sense model has 3 embeddings per word with 300 dimensions each. 
Among multi-sense embedding models we use Multi-Sense Skip-gram (MSSG) \cite{neelakantan2014efficient}, Multi-prototype Skip-gram (MPSG) \cite{tian2014probabilistic}, AdaGram \cite{bartunov2016breaking} and MUSE \cite{lee2017muse}. 

We report the score for the best performing model from each method in Table \ref{tab:scws}.
For MUSE, the best model (Boltzmann method) is used with the trained weights  published in https://github.com/MiuLab/MUSE.
Our sense embedding model is competitive in AvgSimC measure whereas the knowledge distillation method significantly improves the MaxSimC score.
We can infer from this result that the improvement in sense induction mechanism helped learn better embeddings for each word sense.
We can see that best performing multi-sense embedding model's performance is very close to the 900 dimensional skip-gram embeddings (69.3 vs 68.4).
The best performing multi-sense model considering the average over the 2 measures is MUSE with an average of 68.2.
But it does not do well on the word sense induction task.
This indicates that this word similarity task is not very effective at evaluating the performance of word sense embedding models as stated in \cite{bartunov2016breaking}.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c} \hline 
    Model & AvgSimC & MaxSimC \\ \hline
    Skip-Gram (300D) & $65.2$ & $65.2$ \\
    Skip-Gram (900D) & $68.4$ & $\mathbf{68.4}$ \\ \hline \hline
    MSSG & $\mathbf{69.3}$ & $57.26$ \\ 
    MPSG & $65.4$ & $63.6$ \\ 
    AdaGram & $61.2$ & $53.8$ \\
    MUSE & $68.8$ & $67.6$ \\ \hline \hline
    SenseEmbed & $67.6$ &  $54.7$ \\
    BertSense & $62.6$ & $64$ \\
    BertKDEmbed & $68.6$ & $67.2$ \\ \hline
    \end{tabular}
    \caption{Spearman rank correlation score ($\rho \times 100$) on the SCWS dataset. Skip-gram is the only single-sense embedding model. All other embedding models are 300 dimensional. Skip-gram results are reported in \cite{bartunov2016breaking}, MUSE score is obtained using their published model weights and for other models the results are from the respective papers.}
    \label{tab:scws}
\end{table}

\subsection{Effectiveness of Knowledge Distillation}
We can use the intermediate sense embeddings $\{\mathbf{u}_i^1, \dots, \mathbf{u}_i^K\}$ from the Bert sense model on word sense induction and contextual word similarity tasks.
This model does not learn global embeddings.
So we cannot use Eq. \ref{eq:c} to get context embedding for a word in context. 
Since the Bert sense embeddings are trained using the output embeddings from Bert, we can use them instead.

In the knowledge distillation method, we train our sense embedding model to mimick the sense distribution from the Bert sense model.
Since the word sense induction task evaluates the predicted sense of the model, this is the ideal task to quantify the quality of knowledge transfer from Bert to the sense embedding model.
The Bert sense model is compared with the sense embedding model trained with knowledge distillation in Table \ref{tab:kd-wsi}. 
As the Bert sense model is trained with MSE (Mean Squared Error) loss, it's sense embeddings have the same dimensionality as Bert (768).
So we can achieve from $75\%$ to $88\%$ ARI scores with the 300 dimensional embedding model while removing the 12 layer transformer model with 768 dimensional embeddings.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c} \hline
    Model & SE-2007 & SE-2010 & SE-2013 \\ \hline
    BertSense & $0.195$ & $0.163$ & $0.155$ \\ \hline
    BertKDEmbed & $\mathbf{0.145}$ & $\mathbf{0.144}$ & $\mathbf{0.133}$ \\ \hline
    \end{tabular}
    \caption{Word sense induction using the Bert sense model (768D) and knowledge distilled sense embedding model (300D). ARI (Adjusted Rand Index) scores are reported.}
    \label{tab:kd-wsi}
\end{table}

We also compare the Bert sense model with the sense embedding model on the contextual word similarity task in Table \ref{tab:kd-scws}.
The lower correlation score from Bert sense model indicates that these embeddings are not better at sense representation although they remarkably learn to disambiguate senses.
The loss function in Eq. \ref{eq:L_bert} effectively encourages the model to learn linear components of the Bert output embeddings and use them to represent the senses of a word.
Although this helps the model to extract the sense information contained in the Bert output embeddings, this is not the optimal representation for word senses.
The sense embedding model combined with the knowledge gained from the Bert sense model learns to do both i) sense selection and ii) sense representation effectively.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c} \hline 
    Model & AvgSimC & MaxSimC \\ \hline
       BertSense & $62.6$ & $64$ \\ \hline
       BertKDEmbed & $68.6$ & $67.2$ \\ \hline
    \end{tabular}
    \caption{Comparison of Bert sense model with sense embedding trained with knowledge distillation. Spearman rank correlation ($\rho \times 100$) scores are reported on the SCWS dataset.}
    \label{tab:kd-scws}
\end{table}

